VATT: Transformers for Multimodal Self-Supervised Learning from Raw Video, Audio and Text

We present a framework for learning multimodal representations from unlabeled data using convolution-free Transformer architectures. Specifically, our Video-Audio-Text Transformer (VATT) takes raw signals as inputs and extracts multimodal representations that are rich enough to benefit a variety of downstream tasks. We train VATT end-to-end from scratch using multimodal contrastive losses and evaluate its performance by the downstream tasks of video action recognition, audio event classification, image classification, and text-to-video retrieval. Furthermore, we study a modality-agnostic, single-backbone Transformer by sharing weights among the three modalities. We show that the convolution-free VATT outperforms state-of-the-art ConvNet-based architectures in the downstream tasks. Especially, VATT's vision Transformer achieves the top-1 accuracy of 82.1% on Kinetics-400, 83.6% on Kinetics-600, 72.7% on Kinetics-700, and 41.1% on Moments in Time, new records while avoiding supervised pre-training. Transferring to image classification leads to 78.7% top-1 accuracy on ImageNet compared to 64.7% by training the same Transformer from scratch, showing the generalizability of our model despite the domain gap between videos and images. VATT's audio Transformer also sets a new record on waveform-based audio event recognition by achieving the mAP of 39.4% on AudioSet without any supervised pre-training. VATT's source code is publicly available.

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see Section~\ref{sec:conclusion} Conclusion and Discussion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please see Section~\ref{sec:conclusion} Conclusion and Discussion.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We still need time to clean up the code and secure peer reviews before releasing the code.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please see the main text and the appendices.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Because of the computation costs, we did not run the experiments multiple times.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? 
    \answerYes{} Please see Section~\ref{sec:exp_setup}, Table~\ref{table:video-classification-all}, and Table~\ref{table:drop-token-acc-pre-train}.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We used publicly available datasets whose licenses allow research usage. For the HowTo100M~\cite{howto100m} dataset, we additionally comply with Youtube's policies and used only a subset of it.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{To the best of our knowledge, the data we used contains no personally identifiable information or offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/audio_event_classification.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{@{}lcccc@{}}
    \toprule
        \sc Method & mAP & AUC & d-prime \\
    \midrule
    DaiNet~\cite{dai2017very} & 29.5 & 95.8 & 2.437\\
    LeeNet11~\cite{lee2017sample} & 26.6 & 95.3 & 2.371\\
    LeeNet24~\cite{lee2017sample} & 33.6 & 96.3 & 2.525\\
    Res1dNet31~\cite{kong2020panns} & 36.5 & 95.8 & 2.444\\
    Res1dNet51~\cite{kong2020panns} & 35.5 & 94.8 & 2.295\\
    Wavegram-CNN~\cite{kong2020panns} & 38.9 & 96.8 & 2.612\\
    \midrule
    \ours-Base & \textbf{39.4} & \textbf{97.1}  & \textbf{2.895}\\
    \midrule
    \ours-MA-Medium & 39.3 & 97.0  & 2.884\\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Results for audio event classification on AudioSet.}
    \label{table:audio-classification}
\end{table}

==> tables/image_classification.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{@{}lccc@{}}
    \toprule
        \sc Method & \sc Pre-training data & \sc Top-1 & \sc Top-5 \\
        
    \midrule
    iGPT~\cite{chen2020generative} & ImageNet & 66.5 & - \\
    ViT-Base~\cite{dosovitskiy2021an} & JFT & \textbf{79.9} & - \\
    \midrule
    \ours-Base & - & 64.7 & 83.9 \\
    \ours-Base & HowTo100M & 78.7 & 93.9\\
    \bottomrule
    \end{tabular}
    \vspace{1mm}
    \caption{Finetuning results for  ImageNet classification.}
    \label{table:image-classification}
    \vspace{-4mm}
\end{table}

==> tables/video_action_recognition.tex <==
\begin{table}[h]
    \begin{minipage}[h]{0.4\textwidth}
    \small
    \centering
    \begin{tabular}{@{}lcccc@{}}
    \toprule
        \sc Method & \sc Top-1 & \sc Top-5 & \sc TFLOPs\\
    \midrule
    %ARTNet~\cite{} & 69.2 & 88.3 & 6.0\\
    I3D~\cite{carreira2017quo} & 71.1 & 89.3 & -\\
    R(2+1)D~\cite{du2017r2+1d}  & 72.0 & 90.0 & 17.5\\
    MFNet~\cite{lee2018motion} & 72.8 & 90.4 & -\\
    Inception-ResNet~\cite{alom2020improved} & 73.0 & 90.9 & -\\
    bLVNet~\cite{fan2019blvnet} & 73.5 & 91.2 & 0.84\\
    $A^2$-Net~\cite{chen20182} & 74.6 & 91.5 & -\\
    TSM~\cite{lin2019tsm} & 74.7 & - & -\\
    S3D-G~\cite{xie2018rethinking} & 74.7 & 93.4 & -\\
    Oct-I3D+NL~\cite{chen2019drop} & 75.7 & - & 0.84\\
    D3D~\cite{stroud2020d3d} & 75.9 & - & -\\
    GloRe~\cite{glore} & 76.1 & - & -\\
    I3D+NL~\cite{wang2018nonlocal} & 77.7 & 93.3 & 10.8\\
    ip-CSN-152~\cite{tran2019video} & 77.8 & 92.8 & -\\
    MoViNet-A5~\cite{kondratyuk2021movinets} & 78.2 & - & 0.29 \\
    CorrNet~\cite{corrnet} & 79.2 & - & 6.7\\
    LGD-3D-101~\cite{lgdnet} & 79.4 & 94.4 & -\\
    SlowFast~\cite{slowfast} & 79.8 & 93.9 & 7.0\\
    X3D-XXL~\cite{feichtenhofer2020x3d} & 80.4 & 94.6 & 5.8\\
    TimeSFormer-L~\cite{bertasius2021space} & 80.7 & 94.7 & 7.14\\
    %ViViT-Large~\cite{vivit} & 81.3 & 94.7 & 47.90\\
    \midrule
    \ours-Base & 79.6 & 94.9 & 9.09\\
    \ours-Medium & 81.1 & \textbf{95.6} & 15.02\\
    \ours-Large & \textbf{82.1} & 95.5 & 29.80\\
    \midrule
    \ours-MA-Medium & 79.9 & 94.9 & 15.02\\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Video action recognition accuracy on Kinetics-400.}
    \label{table:video-classification-k400}
    \vspace{-2mm}
    \end{minipage}\hfill{}%
    \begin{minipage}[h]{0.45\textwidth}
    \small
    \centering
    \begin{tabular}{@{}lccc@{}}
    \toprule
        \sc Method & \sc Top-1 & \sc Top-5 \\
    \midrule
    I3D-R50+Cell~\cite{wang2020attentionnas} & 79.8 & 94.4\\
    LGD-3D-101~\cite{lgdnet} & 81.5 & 95.6\\
    SlowFast~\cite{slowfast} & 81.8 & 95.1\\
    X3D-XL~\cite{feichtenhofer2020x3d} & 81.9 & 95.5\\
    TimeSFormer-HR~\cite{bertasius2021space} & 82.4 & 96.0\\
    MoViNet-A5~\cite{kondratyuk2021movinets} & 82.7 & 95.7 \\
    %ViViT-Large~\cite{vivit} & 83.0 & 95.7 \\
    \midrule
    \ours-Base & 80.5 & 95.5 \\
    \ours-Medium & 82.4 & 96.1 \\
    \ours-Large & \textbf{83.6} & \textbf{96.6} \\
    \midrule
    \ours-MA-Medium & 80.8 & 95.5 \\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Video action recognition accuracy on Kinetics-600.}
    \label{table:video-classification-k600}
    \vspace{-2mm}

    \small
    \centering
    \begin{tabular}{@{}lccc@{}}
    \toprule
        \sc Method & \sc Top-1 & \sc Top-5 \\
    \midrule
    TSN~\cite{wang2016temporal} & 25.3 & 50.1\\
    R3D-50~\cite{ryoo2019assemblenet} & 27.2 & 51.7\\
    TRN~\cite{zhou2018temporal} & 28.3 & 53.4\\
    I3D~\cite{carreira2017quo} & 29.5 & 56.1\\
    blVNet~\cite{fan2019more} & 31.4 & 59.3\\
    SRTG-R3D-101\cite{stergiou2021learn} & 33.6 & 58.5\\
    AssembleNet-101~\cite{ryoo2019assemblenet} & 34.3 & 62.7\\
    %ViViT-Large~\cite{vivit} & 38.0 & 64.9 \\
    MoViNet-A5~\cite{kondratyuk2021movinets} & 39.1 & - \\
    \midrule
    \ours-Base & 38.7 & 67.5 \\
    \ours-Medium & 39.5 & \textbf{68.2} \\
    \ours-Large & \textbf{41.1} & 67.7 \\
    \midrule
    \ours-MA-Medium & 37.8 & 65.9 \\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Video action recognition accuracy on Moments in Time.}
    \label{table:video-classification-mit}
    \vspace{-6mm}
    \end{minipage}
\end{table}


==> tables/zero_shot_retrieval.tex <==
\begin{table}[h!]
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{@{}lccccccc@{}}
    \toprule
        & & & \multicolumn{2}{c}{YouCook2} &  \multicolumn{2}{c}{MSR-VTT}\\ \cline{4-5} \cline{6-7}
        \sc Method & \sc Batch & \sc Epoch & R@10 & MedR & R@10 & MedR \\
        \midrule
    MIL-NCE ~\cite{miech2020end} & 8192 & 27 & \textbf{51.2} & \textbf{10} & \textbf{32.4} & \textbf{30} \\
    MMV ~\cite{mmv} & 4096 & 8 & 45.4 & 13 & 31.1 & 38 \\
    \midrule
    %\ours-MBS & 8192 & 6 & \textbf{51.2} & \textbf{10} & 29.2 & 42 \\
    \ours-MBS & 2048 & 4 & 45.5 & 13 & 29.7 & 49 \\
    \midrule
    \ours-MA-Medium & 2048 & 4 & 40.6 & 17 & 23.6 & 67 \\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Zero-shot text-to-video retrieval. We evaluate our text and video Transformers of the final pre-training checkpoint.}
    \label{table:retrieval} 
    \vspace{-2mm}
\end{table}
